Implicit Rate-Constrained Optimization of Non-decomposable Objectives

We consider a popular family of constrained optimization problems arising in machine learning that involve optimizing a non-decomposable evaluation metric with a certain thresholded form, while constraining another metric of interest. Examples of such problems include optimizing the false negative rate at a fixed false positive rate, optimizing precision at a fixed recall, optimizing the area under the precision-recall or ROC curves, etc. Our key idea is to formulate a rate-constrained optimization that expresses the threshold parameter as a function of the model parameters via the Implicit Function theorem. We show how the resulting optimization problem can be solved using standard gradient based methods. Experiments on benchmark datasets demonstrate the effectiveness of our proposed method over existing state-of-the art approaches for these problems. The code for the proposed method is available at https://github.com/google-research/google-research/tree/master/implicit_constrained_optimization .

==> conclusion.tex <==
\section{Conclusion}


==> refinements.tex <==
\section{Refinements and Extensions}
\label{sec:refinements}
We close by highlighting how our proposal can be  extended to handle more complex settings and constraints.
\subsection{Inequality constraints}
All the metrics described so far are defined with equality constraints. In our current implementation, we handle inequality constraints by searching for thresholds that satisfy the original non-smooth inequality constraints (during the correction step in Algorithm \ref{algo:implicit} and finally at the end of training). However, we can easily extend our proposal to  handle inequality constraints of the form $\tg(\theta,\lambda)\leq \0$ in a more principled manner.
In this case, we will introduce $m$ auxiliary slack variables $\xi_1,\ldots,\xi_m \in \R_+$, and rewrite the inequality-constrained problem as one with equality constraints:
\begin{align}
\min_{\theta \in \R^p, \xi\in \R^m_+} \tf(\theta,\lambda) \quad \text{s.t. } \tg(\theta,\lambda) + \xi = \0.
\label{eq:opt-inequality}
\end{align}
We can now apply  Algorithm \ref{algo:implicit} to solve the re-written problem by treating the model parameters and auxiliary variables $(\theta, \xi) \in \R^p \times \mathbb{R}^m_+$ together as the optimization variables, with an additional projection step in the gradient descent procedure to ensure non-negativity of the $\xi_i$s.
\subsection{Fairness constraints}
Our approach can also be used to optimize for more recent group fairness metrics \cite{zafar2017fairness}. In a typical fairness setup, each example belongs to one of $m$ protected groups, and the goal is to constrain the model to have equitable performance across all groups. On way to enforce this requirement is to introduce a threshold $\lambda_i$ for examples from group $i \in [m]$, and to then tune the $m$ thresholds to satisfy the fairness constraints \cite{hardt2016equality}. This reliance upon thresholds makes these constraints amenable to optimization with implicit functions.
For example, if one wishes to minimize the classification error subject to the 80\% rule \cite{biddle2006adverse}, which requires the proportion of positive predictions to be at least 80\% for each group, one can set this up as an optimization problem of the form \eqref{eq:opt-inequality}, with the objective $f$ defined as the classification error, and the constraints set to:
\[
g_i(\theta,\lambda) \,=\,  \frac{1}{m_i}\left({\tp_i(s^\theta_{\lambda_i}) + \fp_i(s^\theta_{\lambda_i})}\right) - 0.8,
\]
where $\tp_i$ and $\fp_i$ are the true positives and false positives on examples belonging group $i$, and $m_i$ is the total number of examples in group $i$. In practice, one can impose more than one constraint per group, as long as for any $\theta$, one can always find  thresholds $\lambda_i$s for which the constraints are satisfied (which is indeed the case with  popular fairness metrics such as equal opportunity \cite{hardt2016equality}).

\subsection{Multi-class metrics}

In our experiments, we handled multi-label classification tasks. The extension to multi-class metrics requires some effort as in this case we are allowed to predict only one among $m$ labels. As with the multi-label setting, we work with a model $s^\theta: X \> \R^m$ that outputs $m$ scores, and we will maintain one parameter $\lambda_i$ for each label $i \in [m]$. The parameters  $\lambda_i$'s would then be used to post-shift the model via a \textit{weighted argmax} to predict the final class:
\[
s^\theta_\lambda(x) \in \argmax_{i \in [m]} \lambda_i s^\theta_i(x).
\]
Computing the parameters $\lambda$s so that the resulting classifier satisfies the specified constraints is not straightforward, but can still be performed efficiently with e.g.\ the methods in \citet{narasimhan2015consistent}. While it isn't clear if a feasible $\lambda$ exists for general rate constraints, it certainly does for constraints like ``coverage'' \cite{cotter2019optimization}, which require that the model makes a certain percentage of predictions from each class.


\subsection{Ranking metrics}

Perhaps, the most interesting extension of our approach is to query-based ranking problems \cite{schutze2008introduction}, where each example contains a query and a list of documents, and the goal is to rank the documents based on the relevance to the query. Popular ranking metrics such as Precision@$K$ or Recall@$K$ seek to measure performance in the top ranked documents \cite{lapin2017analysis}. Unfortunately, writing these metrics out as an explicit constrained optimization problem would require one constraint per query, with the number of constraints growing with the size of the training set. Consequently, standard constrained optimization approaches, when applied to optimize these metrics, would need to maintain one Lagrange multiplier for each query, making it impractical to use them with large datasets. Recently, \cite{narasimhan2020} propose solving such heavily-constrained problems with lower-dimensional representations of Lagrange multipliers. In contrast, our method offers an alternate route which does not require explicitly handling the large number of constraints, through implicit modeling of the per-query thresholds. We look forward to future work comparing our implicit thresholding approach with the state-of-the-art  methods for these ranking metrics (e.g. \citet{kar2015surrogate,lapin2017analysis}).

